Weingarten Calculus

We consider the problem of computing the integral $$ \int_{\mathcal{U}(d)} u_{i_1j_1}\cdots u_{i_nj_n} \bar{u}_{i'_1j'_1} \cdots \bar{u}_{i'_{n'}j'_{n'}} dU, $$ where the integration takes place with respect to the probability Haar measure on the unitary group $\mathcal{U}(d)$, and the $u_{ij}$ denotes the $ij$-th entry of a unitary matrix $U$. We present a unified approach connecting classical results, the explicit formula for the integral given by B. Collins and P. Sniady and subsequent works of various authors providing different points of view. Finally we are able to provide an explicit formula for the $2n$-th moment of the trace of a unitary Haar random matrix, generalizing a result of P. Diaconis.

==> frontbackmatter/danksagung.tex <==
\pdfbookmark[1]{Danksagung}{Danksagung}
% \addcontentsline{toc}{chapter}{\tocEntry{Abstract}}

\begingroup
\let\clearpage\relax
\let\cleardoublepage\relax
\let\cleardoublepage\relax

\chapter*{Danksagung}
Ich möchte mich bei Herrn Professor Franz Lehner für seine Geduld, seine zahlreichen Vorschläge und dafür, dass er mir ein so spannendes und abwechslungsreiches Themenfeld näherbrachte, bedanken.
\vspace{1em}

Weiters bedanke ich mich bei meinen Freunden und Studienkollegen, mit denen selbst die größte Anstrengung Spaß machte.

\vspace{1em}
Zu guter Letzt möchte ich meiner Familie danken. Ohne ihre tatkräftige  Unterstützung gäbe es diese Arbeit wohl nicht. 
% \begin{otherlanguage}{ngerman}
% \pdfbookmark[1]{Zusammenfassung}{Zusammenfassung}
% \chapter*{Zusammenfassung}
% Kurze Zusammenfassung des Inhaltes in deutscher Sprache\dots
% \end{otherlanguage}

\endgroup

\vfill

